"Community Guidelines Make this the Best Party on the Internet": An In-Depth Study of Online Platforms' Content Moderation Policies

Moderating user-generated content on online platforms is crucial for balancing user safety and freedom of speech. Particularly in the United States, platforms are not subject to legal constraints prescribing permissible content. Each platform has thus developed bespoke content moderation policies, but there is little work towards a comparative understanding of these policies across platforms and topics. This paper presents the first systematic study of these policies from the 43 largest online platforms hosting user-generated content, focusing on policies around copyright infringement, harmful speech, and misleading content. We build a custom web-scraper to obtain policy text and develop a unified annotation scheme to analyze the text for the presence of critical components. We find significant structural and compositional variation in policies across topics and platforms, with some variation attributable to disparate legal groundings. We lay the groundwork for future studies of ever-evolving content moderation policies and their impact on users.

==> sections/related.tex <==
%!TEX root = proposal.tex

\section{Related Work}

\paragraph{Content moderation taxonomies.} Studying content moderation first
requires defining and scoping it.  In prior work, Goldman developed a taxonomy
of content moderation~\cite{goldman2021content}, shown in Figure~\ref{fig:taxonomy}, which we use to
scope our work. Although we use the term {\em content moderation} throughout
the proposal, Goldman's taxonomy highlights that moderation can in fact take
many forms. When we use the term ``content moderation'', we are 
referring to actions by the platforms that Goldman refers to as ``content
regulation''. We use {\em content moderation} to refer to this more
specific set of actions because it is a more widely used term.

\paragraph{Legal research on content moderation.} The importance of
content moderation has spurred a robust legal discussion~\cite{gillespie2018custodians,suzor2019lawless,klonick2017new}.  Three 
questions are outlined in previous work~\cite{goldman2021content,klonick2017new}:
(1)~What content should be allowed online? This question is concerned with the
first amendment. As we discussed in the introduction, the laws are much
clearer for copyright infringement than for misinformation.  (2)~Who should
make the substantive rules of online content and activities?
Klonick~\cite{klonick2017new} further distinguishes standards (e.g., ``don't drive too
fast'') from rules (e.g., ``a speed limit set at sixty-five miles per hour'')
in the current practice of Internet platforms.  (3)~Who should determine if a
rule violation has occurred, and who should hear any appeals of those
decisions?  While existing research is mostly qualitative, our goal is to
examine the rules and audit the moderation practice through measurement
studies, and contrast that with user understanding.  

\paragraph{Content moderation on online communities.} Content moderation has
attracted substantial interest from computer science researchers because of
its growing importance in online communities~\cite{kiesler2012regulating}.
Content moderation can potentially filter ``bad'' content and ``bad'' actors
and promote a healthy community, but may also infringe an individual's right
to freedom of expression.  Thus, there is a large body of research studying
the effect of moderation on community behavior, including whether one should
regulate online content at
all~\citep{Chancellor:2016:TIC:2818048.2819963,chandrasekharan2017you,srinivasan+dnm+lee+tan:19,jhaver2019does,Chang-Recidivism:19,seering_shaping_2017,matias2019preventing,cheng+dnm+leskovec:2014}.
For instance, PI Tan has developed an observational method that leverages
delayed feedback (i.e., content moderation does not happen instantaneously) to
understand the causal effect of comment removal on users' future
behavior~\cite{srinivasan+dnm+lee+tan:19}.

Related to our proposed work, there is a growing line of research on
characterizing the rules on online platforms~\cite{fiesler_reality_2016,
fiesler_reddit_nodate,fiesler_understanding_2015,fiesler_what_2017,
fiesler+al:2018,Brian_keegan_2017,chandrasekharan_internets_2018}.  For
instance, some work~\cite{Brian_keegan_2017} studied the evolution of rules on
Wikipedia by tracking revisions on rule-related Wikipedia pages. In another
study, researchers \cite{fiesler+al:2018} provided a characterization of
different types of rules and show that community rules share common
characteristics across subreddits.  In comparison, other
researchers~\cite{chandrasekharan_internets_2018} performed a large-scale
study to understand content moderation through the language used in the
removed comments on Reddit and identify norms that are universal (macro),
shared across certain groups (meso), and specific to individuals (micro).  
Our work adds to this body of work by understanding
how well the implementation of community rules aligns with the official
language in the terms of service, community standards, and the associated
legal requirements.  We also propose to audit the
outcome of content moderation.
% , independent of the underlying technology or manual effort in
% achieving the outcome of content moderation.  

\paragraph{User understanding of content moderation.}
There is a large growing body of research around how users understand content
moderation and how users react to content moderation. For instance, 
% there are
% numerous studies of how Reddit users react to post-level and community level
% moderation such as quarantining or banning an entire subreddit
numerous studies examine how Reddit users react to post-level and community-level moderation~\cite{jhaver2019does, jhaver_did_2019, jhaver_human-machine_2019,
jhaver_online_2018, matias_going_2016, chandrasekharan_quarantined_nodate,
chandrasekharan_you_2017, chandrasekharan2019crossmod, Copeland:vldb1989,jhaver_evaluating_2021}. For
example, prior work has shown that banning subreddits with hateful speech does
decrease toxicity overall, however, toxicity within the banned subreddit may
increase \cite{chandrasekharan_you_2017, Copeland:vldb1989}.   
% Others studied how deplatforming an individual affects
%  users on Twitter \cite{jhaver_evaluating_2021}. 
In some cases, content
moderation can increase toxicity and move people to more extreme on another
platform \cite{horta_ribeiro_platform_2021}. These studies imply that users
who know about community rules or who received explanations for their removals are often more accepting of moderation
practices \cite{jhaver_did_2019, jhaver2019does}. 

User studies have also studied content moderators themselves
\cite{roberts_commercial_nodate, roberts2014behind, ahmad_its_2019} and compared how users
view user-moderated platforms such as Reddit \cite{jhaver_human-machine_2019, juneja_through_2020, cook_commercial_2021} versus employee-moderated platforms such as Facebook or
Twitter. Researchers have also examined how
users experience to algorithmic content moderation \cite{vaccaro_at_2020} and whether content moderated decisions are politically
motivated \cite{jiang_identifying_2020, jiang_reasoning_2020} as well as less obvious forms of softer forms of content
moderation such as shadow banning
\cite{myers_west_censored_2018, zannettou_i_2021}. Some have also examined how to
make moderation more transparent \cite{suzor_what_2019}. Much of this work
focused on content moderation on one platform, for one type of
online content; our work aims to take a more holistic approach.

\paragraph{Audit studies.} Although computer scientists have made progress on
the recruitment and coordination of testers, the generation of prompts has
remained a manual process.  Social scientists have created externally valid
audit prompts by manually adapting real-world content. In one audit of
employment discrimination, researchers downloaded resumes from an online
website and edited them to create their decision
prompts~\cite{bertrand_are_2004}. In a study of online censorship in China,
researchers looked for news articles about political and non-political
collective action that they then tested posting to Chinese social
media~\cite{king_reverse-engineering_2014}. Perel and Elkin-Koren~\cite{perel2017black} tested the enforcement of copyright rules across several image and video platforms in Israel using manually created probes. They found inconsistent and overly aggressive filtering of material, with non-infringing material often being removed.  Researchers have also studied
advertising on online platforms in various ways.  Ribeiro et al. studied how
the Russian Intelligence Research Agency (IRA) used Facebook's ad targeting
tools to create politically divisive ads before the 2016
election~\cite{ribeiro2019microtargeting}.  Andreou et al. also found that
disclaimers for why a user has received an ad are often incomplete,
misleading, and vague~\cite{andreou2018investigating}.  Researchers who
conduct audit studies must always consider the legal and ethical risks for
four parties: the testers, people who might encounter the prompts, the parties
that oversee the decision-making system, and the
researchers~\cite{pager_use_2007}. Our work will build on these audit studies
to examine online content moderation in practice.

